Characterizing the Identity of Model-based Safety Assessment: A Systematic Analysis

Model-based safety assessment has been one of the leading research thrusts of the System Safety Engineering community for over two decades. However, there is still a lack of consensus on what MBSA is. The ambiguity in the identity of MBSA impedes the advancement of MBSA as an active research area. For this reason, this paper aims to investigate the identity of MBSA to help achieve a consensus across the community. Towards this end, we first reason about the core activities that an MBSA approach must conduct. Second, we characterize the core patterns in which the core activities must be conducted for an approach to be considered MBSA. Finally, a recently published MBSA paper is reviewed to test the effectiveness of our characterization of MBSA.

==> 1_introduction_old.tex <==
\section{Introduction}\label{sec:intro}
Model-based safety assessment\footnote{Sometimes also known as model-based safety analysis.} (MBSA) has been around for three decades. The benefits of MBSA have been well-documented in the literature, such as tackling complexity, introducing formal methods to eliminate the ambiguity in the traditional safety analysis, using automation to replace the error-prone manual safety modeling process and making sure the consistency between the design model and the safety model \cite{prosvirnova2014altarica}. 
Prominent modeling languages such as AADL-EMV2 \cite{larson2013illustrating,procter2020aadl,feiler2017automated}, AltaRica \cite{machin2019modeling, bieber2004safety, mortada2014safety, tlig2018autonomous} and HipHops \cite{kabir2019conceptual, chen2013systems} are generally considered as MBSA, which according to \cite{bozzano2015safety} are the only three languages that “have matured beyond the level of research prototypes”.

MBSA approaches are significantly different in the literature \cite{stewart2021aadl}. We have seen a flourish of research development over the years, but Software Engineering seems to have a stronger presence in the MBSA literature as most of the MBSA innovation focuses on model specification notations and/or algorithms for possible manipulations of the models \cite{lisagor2010illusion}. 
However, there is still a lack of consensus on what MBSA even is. A question such as what makes an approach MBSA is left unanswered. 
For example, is Formal Methods applying to safety analysis MBSA? Does safety analysis even mean the same thing in the context of Formal Methods? 
This ambiguity has significant implications to System Safety Engineering \footnote{System Safety Engineering is a discipline to identify hazards and then to eliminate the hazards or reduce the associated risks when the hazards cannot be eliminated \cite{dod2012mil-std-882e}.}, because it jeopardizes the identity of MBSA as a main research thrust of the System Safety Engineering community. Without a clear definition and boundary, MBSA can quickly become a buzzword that any other disciplines can claim as long as the work uses computer model and is safety-related (e.g., \cite{pajic2012model-driven, althoff2010reachability}). 

Therefore, this paper aims to investigate the identity of MBSA. Specifically, we are asking the following three questions:  
\begin{itemize}
    \item What are the minimal set of requirements for an approach to be MBSA?
    \item What are the possible patterns that each of the requirements is implemented in the literature?
    \item What are the suggestions for MBSA as a line of collective research efforts moving forward? 
\end{itemize}

\paragraph{Research method.}
A common approach to investigate the identity of a research subject is literature review. 
In a conventional review, papers are systematically collected based on a set of pre-defined criteria with respect to the scope of the subject matter. 
However, we do not have that privilege because MBSA is ill-defined. Any pre-defined criteria to decide whether a paper should be reviewed or not will be biased toward the authors' pre-existing view about MBSA. 

As a solution, we start from a broader and better-established scope of MBSA. We refine this scope into a minimal set of well-understood activities that a MBSA approach must absolutely conduct (called ``essential activity'' in this paper). For each essential activity, we classify the literature based on how it is accomplished by different approaches (called ``patterns'' in this paper). After that, we summarize a minimal set of commonalities among the patterns as the minimal set of requirements for an approach to be MBSA. Finally, we give suggestions for the MBSA research moving forward. 

For this reason, we put forward the following assertion:
\vspace{2mm}

\noindent \emph{Assertion: MBSA is Model-based Design (MBD) applied to system safety assessment in a specific way.}

\vspace{2mm}
\noindent Although it is difficult to find direct evidence to support this assertion because there is no consensus on an exact definition of MBSA, this assertion is consistent with \cite{joshi2006model-based} that claims MBSA is an extension of safety analysis to Model Based Design. 
More importantly, our confidence in starting from this assertion is that (1) both MBD and safety assessment are well-defined so that the reasoning process will not be biased towards the authors' pre-existing view about MBSA, and (2) such an assertion is general enough so that we will not miss important characteristics of MBSA by starting off with a too narrow view.
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/venn.pdf}
    \caption{ The venn diagram that summarizes of the research method of this paper. }
    \label{fig:venn}
\end{figure}

Specifically, our approach can be described in a venn-diagram in Fig.\ref{fig:venn}. First, we reason about the set of activities that need to be conducted when MBD is applied to safety assessment. This set is the overlapping area between the blue oval and the green oval of Fig.\ref{fig:venn}. 

Second, we use the identified activities to characterize MBSA. Some or all of the identified activities must be conducted in a specific way so that an approach can be considered as MBSA. 
Therefore, MBSA is a subset of the intersection of MBD and safety assessment (i.e., Area 3 of Fig.\ref{fig:venn}). Note that the decision about which activities that an MBSA approach should conduct is highly judgemental. Therefore, we only \emph{recommend} a minimal set of activities that an approach must take to be considered as MBSA. However, as argued earlier, an exact definition of MBSA is less important than the reasoning process and the rationale behind the decisions about whether an activity should be conducted by MBSA or not. 

Third, we classify current MBSA approaches in terms of how the recommended activities are conducted in the current literature, in order to provide a road map for the safety engineers to evaluate, compare and select the MBSA approach that is the best fit for his/her problem at hand. 

Finally, we identify what current MBSA approaches cannot do for safety assessment, i.e., Area 4 in Fig.\ref{fig:venn}, in order to (1) help the safety engineers avoid over-claiming the safety argument, and (2) help the MBSA methodology developers invent more comprehensive approaches to better accomplish the mission of safety assurance. 


==> 2_background_old.tex <==
\section{Background}\label{sec:background}
\subsection{The model-based approach}

With the increase in system complexity and productivity challenges, model-based design and engineering approaches have become the preferred engineering paradigm in safety critical  applications. Model-based approach supports system requirements, documentation, design, and verification of complex embedded systems throughout the product life cycle from the concept phase to the later development phases \cite{hart2015introduction}.

Over the years, ``model-based'' approaches have been used in different contexts where it’s meaning, and purpose is somewhat unclear. The graphical models in ``Model based'' approaches can serve as software or system prototypes, increasing the overall productivity \cite{mbe}.  Model-Based Systems Engineering (MBSE),  Model-Based Design (MBD),  Model-Based Engineering (MBE) are some of the many ``model-based'' acronyms used in literature. Additionally, there are ``model-driven'' approaches such as Model-Driven Engineering (MDE), Model-Driven Development (MDD), Model-Driven Architecture (MBA) to name a few. The concept in ``Model- driven'' is the model drives the analysis phase in the development process to come up with a complete set of requirements. Model driven paradigms also support traceability of requirements between various development stages, i.e., requirements, model, and implementation \cite{clarifyconcepts}. It is important to clarify these acronym expressions and address any ambiguities before we review MBSA. Below are some of the commonly used model-based and model-driven approaches. 

\paragraph{Model-Based Systems Engineering} Its is a formal methodology that puts model at the center of the system design to support system requirements, design, analysis, verification, and validation of  complex systems \cite{hart2015introduction}. Models support system architecture, traceability with requirements,  and represent organizational process with components and resources needed. 

\paragraph{Model-Based Design or Model-Driven Development} It is a method of understanding a system’s behavior by simulation of a model, which is graphical representations of a physical system. Model-based designs   support model-based testing and other verification activities on executable models, i.e., production level code can automatically be generated from the model \cite{friedman2006matlab}. Further, tools such as MathWorks Simulink and Ansys SCADE also support safety standard compliance checks for the models. 

\paragraph{Model-Based Engineering or Model-Driven Engineering} They are engineering approaches where models are primary artifacts in the development process \cite{liebel2018model}. MBE/MDE approach masks the complexity of a design by using models. MBE emphasizes graphical programming to improve the development time and efficiency throughout the System Development Life Cycle (SDLC) \cite{mbe}.

\paragraph {Model Based Analysis} It aims to identify design flaws early in the development life cycle by comprehensive testing and verification of the model. Design flaws are addressed, and changes incorporated in model iteratively as defects and missing requirements are identified during analysis \cite{johnson2021continual}. 

\paragraph {Model-Driven Architecture} It is an approach to software development built around the Object Management Group (OMG) standard that intends to reduce complexity and costs in software development. The central goal of model-driven architecture is to have portable and reusable designs by expressing specifications using models. Models are used for documenting, design, testing, coverage analysis, deployment, and maintenance \cite{truyen2006fast}.

\paragraph{Model-Based Safety Engineering} It is the integration of safety engineering and system design by using a common system model. The system model is integrated with the fault model to achieve better quality safety analysis with reduced costs \cite{cancila2009sophia} \cite{joshi2006model}. 
Model-Based Safety Analysis – It is a model-based approach to verify the safety of a system by using models that encompass both failure behavior and physical behavior of the system [10]. Automating safety analysis to a certain extent by using common models between system and safety engineers help improve the quality of safety analysis while reducing costs \cite{nigam2018model}.  

\paragraph {Model-Based Safety and Security Engineering} It is the integration of safety and security in models to avoid hazards. In complex cyber physical systems with a wide attack surface, security violation can lead to violation of safety mechanisms resulting in catastrophic events.  Thus, it is important to incorporate both safety and security in system models to facilitate efficient analysis.


\subsection{Model-based design}
First of all, we are aware that MBD is an overloaded term, as numerous papers tried to differentiate it from ``model-driven engineering,'' ``model-driven design,'' and ``model-driven architecture''\cite{whittle2013state,scippacercola2016}. It is not our intention to define these terms. However, we need a clear understanding of MBD to conduct meaningful discussion about the body of literature pertaining to (or not pertaining to) MBSA. Hence, we adopt the process proposed by \cite{jensen2011model-based} as the ``ground truth'' of our discussion. The left of the Fig.\ref{fig:mbd_process} is the proposed MBD process which can be mapped to the detailed 10 steps of \cite{jensen2011model-based} at the right. We explain all the involved steps in this section. 

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/mbd_process.pdf}
    \caption{The MBD process. The arrows of the left can be mapped to the steps to the right (adopted from \cite{jensen2011model-based}).}
    \label{fig:mbd_process}
\end{figure}

Overall, MBD is comprised of two loops: an inner loop and an outer loop. The inner loop conducts design based on computational models operating in the virtual environment, and the outer loop continues the design by building systems that operate in the real environment to make sure the design decisions made during the inner loop are valid.  

\paragraph{The inner loop.} An MBD process starts with a problem statement (Step A) which details the goal of the design activities, such as a set of functions with performance requirements and safety constraints. 
Second, an engineering solution is derived based the engineer’s domain knowledge. Although 3 independent steps (Step B, C, D) are identified by \cite{jensen2011model-based}, we acknowledge this process in reality can be quite fuzzy, because the engineer’s thought process varies from person to person, depending on their own expertise and nature of the problem at hand. Nevertheless, we prescribe the process always ends with a solution (valid or not) to the stated problem from the perspective of the specific engineering discipline. 
Third, a modeling language is selected to faithfully represent the engineering solution with a model of computation (Step E). Compared to a simulation model that is to loosely ``get a feel'' of the proposed engineering solution, the model in MBD is a faithful computational copy of the engineering solution and hence used as the primary artifact \cite{liebel2014assessing}. Models in MBD are directly evolved into full-fledged implementations without changing the engineering medium, tools, or methods \cite{france2007model-driven}. Specifications and even software code of the implementation are (automatically) derived from the model \cite{larsen2016integrated, hutchinson2011empirical}. Therefore, the modeling language must be fully equipped to express the engineering solution.  
Fourth, Step G closes the inner loop by automatically analyzing the model of computation in order to gain a required level of confidence of the engineering solution before building the prototype or the actual system. 

\paragraph{The outer loop.} Given the model of computation, specification is derived (Step F); hardware is constructed in accordance with the specification (Step H); software is developed or automatically generated from the model and synthesized with the hardware (Step I). This is what makes the ``model'' in MBD different from models for simulation, because 1) specifications for constructing a prototype of the actual system are derived from the model, for example a CATIA model can be used for both structural analysis and directly as 3D drawings for manufacture \cite{manjunath2013structural}, and 2) software code sometimes can even be automatically generated from it, which is the perhaps the main reason for MBD’s growth of popularity in the first place \cite{bhatt2005model-based}.    
Finally, Step J closes the outer loop. The prototype or the actual system is built to verify the engineering solution, and eventually validate the resulting system against the problem statement made at the beginning of the MBD process. 

==> 4_feature_old.tex <==
\section{The notable patterns and the defining features of the essential activities}\label{sec:feature}
In this section, we further reason about the essential activities to develop an in-depth understanding of MBSA. 
For each essential activity, we classify the different ways that the activity is conducted in the literature. The resulting classifications are the notable patterns of MBSA, and the commonalities among the notable patterns are the defining features of MBSA.
An approach must exhibit all the \textbf{defining features} to be considered as MBSA, and a subset of the \textbf{notable patterns} can always be found in an approach that is considered MBSA.  

\subsection{Component fault characterization (Arrow 3)}\label{sec:fault}
This activity is to depict the individual component faults that identified by the deductive analysis (Arrow 2). 
\subsubsection{A unifying model of component fault}
Characterizing component faults is a matter of modeling, and any model is an abstraction of the phenomenon being modeled. Therefore, the question is what information needs to be captured to  characterize a component fault. On one hand, as we will explain in Section \ref{sec:modeling}, the answer to this question depends on the specific analysis to be conducted on the model. A very abstract description of a component fault may be sufficient if the analysis does not require precise estimation. \cite{gudemann2010quantitative} demonstrated that a safety analysis on the same system with different failure models (fault tree vs. failure automata with stochastic dependencies modeling capabilities) results in completely different conclusions, where the results from the fault tree are ``very coarse'' compared to the failure automata introduced in that work.  



On the other hand, the information needed to characterize a component fault also depends on how the component actually fails. 
Unlike other scientific communities such as aerodynamics and heat transfer where the fundamental attributes of the subject phenomenon are well studied, the safety community does not have much fundamental study on the mechanism of component fault as a general scientific phenomenon. 
More often, safety engineers decide the necessary information to characterize a component fault in an ad-hoc way, which makes it challenging to assure the sufficiency of the modeling of component faults. 

Therefore, a more fundamental question is, how a component actually fails. 

This is a very challenging question, because it requires a generic characterization of how any component fails. We are not aware of any first principle that can succinctly generalize such a process. As a result, our solution is to generalize the modeling languages\footnote{We mean modeling language loosely by a pre-defined construct (formal or informal) that can depict a component fault in whatever level of abstraction. }.  
Almost all the modeling languages that can characterize component faults have underlying models (explicit or implicit) of how a component fails, and each of those underlying models is a subset of all the possible ways that a component may fail.  
The idea is that if we can unify the underlying models of as many modeling languages as possible in the literature that can characterize component faults, then the resulting model can be considered as a generic model to characterize the component fault.  

In the rest of Section \ref{sec:fault}, we will propose such a unifying model based on a set of modeling languages we found in the literature.\textbf{ As a caveat}, we do not claim all the modeling languages in the literature are found and reflected in our current unifying model. Instead, we emphasize such a unifying model is a living artifact. As more and more modeling languages are reflected in it, this unifying model gets closer and closer to be a true generic model of how a component fails.   
\subsubsection{The structure of the unifying model}
We propose a structure to characterize component faults in this subsection. 
 All the modeling languages will be interpreted based on this structure, and eventually weaved into 
the unifying model of component faults in the next subsection.

\cite{ericson2015hazard} decompose hazard into three elements: Hazardous Element, Initiating Mechanism and Target/Threat, where Hazardous Element is the basic hazardous resource creating the impetus for the hazard; Initiating Mechanism is the trigger or initiator event(s) causing the hazard to occur through the actualization or transformation of the hazard from a dormant state to an active mishap state; Target/Threat is the mishap outcome and the expected consequential damage and loss. 
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/fault.pdf}
    \caption{At the top is the underlying structure to characterize a component fault. It can be mapped to the three elements of hazard defined by \cite{ericson2015hazard} at the bottom. The solid arrow represents the causal sequence of how a fault/hazard develops.}
    \label{fig:fault}
\end{figure}

Inspired by Ericson's hazard characterization, we propose an underlying structure in Fig. \ref{fig:fault} to characterize component faults. Specifically, the Hazard Element in Ericson's hazard characterization is defined as casual factor in our structure. Each fault is correlated with a set of casual factors, all of which have to be present for the fault to happen. Furthermore, the Initiating Mechanism in Ericson's hazard characterization is decomposed into the activation mechanism and the impact mechanism in our structure. This is driven by the fact that a fault does not necessarily lead to a failure \cite{arp4754a2010guidelines}, implying two processes in play: one leading to the fault (i.e. the activation mechanism) and the other leading to the effect of the fault (i.e. the impact mechanism). Finally, the Target/Threat in Ericson's hazard characterization is defined as the effects on the respective components. In fact, \cite{ortmeier2007formal} also proposed to “split the (fault) process into two parts: one part is modelling how and when the failure occurs and the other is to model the direct, local effects of the failure”, where the first part corresponds to the ``causal factor'' and the ``activation mechanism'', and the second part corresponds to the ``impact mechanism'' and the ``effects'' in our structure.
As a result, a fault is present only when certain conditions are satisfied, and it takes additional conditions for the fault to show effects on the component. This characterization of fault is consistent with the fault propagation process proposed by \cite{avizienis2004basic}. Note that ``fault'' in our paper means “error” in \cite{avizienis2004basic}.

\subsubsection{The notable patterns}
The structure defined previously defines four aspects to characterize component faults. 
In this subsection, we examine the literature for the different ways to implement each aspect.

\paragraph{Causal factors.}
While the specific contents of casual factors vary from application to application, two questions are always addressed in the literature about the causal factors: (1) what causes the fault (i.e., the source) and (2) what is the likelihood of causes (i.e., the occurrence).

The \textbf{source} of the causal factor can be classified with respect to the boundary of the component. As pointed out by \cite{papadopoulos1999hierarchically}, the component fault can be caused by internal causes or external causes. They are the two most common sources of fault addressed in the literature \cite{stewart2017architectural,bozzano2011safety,delange2014aadl}. The difference between the two types of sources are self-explanatory. 

Moreover, the external causes can be further classified into intended and unintended. The intended external causal factor means the intended input becomes erroneous and  causes the fault of the component. For example, a voltage (i.e. the input) too high can break a capacitor in the circuit. A processor depends upon the functioning of a fan and if the fan fails, the processor overheats and fails as well.  Similar concepts can be found in \cite{boudali2008architectural,walter2008opensesame}.

The unintended external causal factor is caused by the secondary effect of a fault stemming from an external component that is not supposed to have interaction with the current component in nominal conditions. \cite{joshi2007behavioral} coins this type of causal factor as ``unconnected'' with an example of two redundant sets of
pipes that are routed very close to each other. A failure of one
of the pipes (say, a pipe burst) can affect the pipe that is routed close to it. In fact, this type of causal factors is very similar to the causal factors addressed in Zonal Safety Analysis and Particular Risk Analysis defined in \cite{arp47611996guidelines}.  
Very few approach in the literature makes an explicit distinction between the intended and the unintended causal factors. We argue that such a distinction is important because (1) the methodology developer must make sure their modeling language can model both phenomenon as they are inherently different in nature, and (2) identifying the unintended external causal factors is challenging, and without explicitly emphasizing it in the modeling language, these causal factors can be easily overlooked by the safety engineers. 




The way to characterize the \textbf{occurrence} of component fault depends on the sources of the causal factors. 
For the external causal factors, the occurrence depends on the source component(s), hence is “propagated”. For the internal causal factors, their occurrence can be probabilistic and Boolean. The probabilistic occurrence is characterized with probability distributions, based on which both quantitative and qualitative safety analysis can be conducted \cite{gudemann2010framework}. The Boolean occurrence depicts the causal factor is present or not, based on which only the qualitative safety analysis can be conducted. The implication is quite straightforward: if quantitative analysis is required, then the occurrence of the internal causal factor has to be characterized with probability distribution; otherwise a Boolean occurrence will suffice. 


\paragraph{Activation mechanism.}
The causal factors being present is the necessary but not sufficient condition for the fault to be present. Activation mechanism is the additional condition  (if applicable) that the causal factors must satisfy to activate the fault, given all the causal factors are present. We examined the literature and obtained the following list of patterns for the activation mechanism.
\begin{itemize}
    \item Guard: The component may be vulnerable to the causal factor(s) only when it is in certain states. For example, overcurrent can cause an electric device to fail only when the device is on. This is a very common phenomenon and is well-understood by the literature.
    \item Sequence: The causal factors may have to happen in a certain sequence so that the fault can be activated. This is one of the main advancements of Dynamic Fault Tree over the traditional FTA.
    \item Delay: It may take time for the fault to happen even after the causal factors are all present. For example, a pump overheats after no water flows in for a certain period of time. This time period can be a deterministic one or a probabilistic one \cite{prosvirnova2013altarica}. A special case is the zero-delay, where the fault is activated right after the causal factors are present. The presence of the causal factors in the zero-delay case can usually be modelled as a trigger event of the fault \cite{kaiser2007state/event}.
    \item Duration: A duration may be defined to model the phenomenon that a fault can be deactivated. A fault can disappear a certain period of time after the activation because of its transient nature \cite{ortmeier2005deductive} or after being repaired \cite{chaux2011qualitative}. A infinite long duration means the fault is permanent. The characterization of the time can be deterministic, probabilistic \cite{ortmeier2005formal} or non-deterministic as suggested by \cite{gudemann2010probabilistic}. 
\end{itemize}

\paragraph{Impact mechanism.}
The fault being present is the necessary but not sufficient condition for the fault show effects on the component. The impact mechanism is the additional condition (if applicable) that needs to be satisfied for a given fault to cause the defined effects. We examined the literature
and obtained the following list of patterns for the activation
mechanism.
\begin{itemize}
    \item Guard: The fault may lead to the defined effects only when the system in certain state. For example, loss of hydraulic supply will only affect the ground deceleration function when the aircraft is the state of landing.  Guard condition is widely modeled in the literature such as in state/event fault tree \cite{kaiser2007state/event} and AltaRica Data-flow \cite{seguin2007formal}. 
    \item Delay: As pointed of by \cite{lisagor2010failure}, “the effect of a failure may not immediately cause an output failure mode and may remain dormant”. The time between the fault being present and the appearance of the fault effect is defined as “Fault Tolerant Time Interval” by \cite{gonschorek2019integrating}. This delay is considered as “safety-relevant properties” in SafeDeML \cite{gonschorek2019safedeml}.
    \item Determinism: It may also be uncertain to determine the exact effects of a fault due to either epistemic uncertainty or aleatoric uncertainty. This uncertainty is traditionally addressed by modeling the worst-case scenario instead of the uncertain process. Not much literature has an non-deterministic impact mechanism. \cite{braman2009probabilistic} coins it as “probabilistic transition conditions”. \cite{delange2014architecture} provides a feature called “branching transition” where multiple target states can be transitioned to following certain probability distribution from one source state. Although this feature was originally designed for branching transient and persistent failure, but it also seems to have the potential to capture the uncertainty of the impact process. 
\end{itemize}

Note that the guard and the delay are defined in both the activation mechanism and the impact mechanism. In most literature, they can even be modeled with the same modeling construct. However, they are inherently different in terms of their respective roles in the component fault as a phenomenon. It is crucial to identify them correctly when characterizing the component faults and then model them accordingly with whatever modeling language selected. 

\paragraph{Effects on the component.}
Effects of a fault on the respective component is modelled differently in the literature. We are able to summarize the patterns in Fig.\ref{fig:effect}.
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.69\linewidth]{figs/effect.pdf}
    \caption{Notable patterns to model the fault effects on a component. A detailed classification of a sample pool of the literature is given in the Appendix.}
    \label{fig:effect}
\end{figure}

As shown in Fig. \ref{fig:effect}, two dimensions are identified from the literature: the abstraction and the semantics. The abstraction dimension determines how many details are included in the effect model. For the component level, the fault affects the internal behaviors of a component. This is also called white box error model in \cite{cuenot2014applying,fenelon1992new}. For the architecture level, the fault effects are represented at the output port of a component and propagated to the input port of other components. This is also called black box error model in \cite{cuenot2014applying,fenelon1992new}. For the function level, the component is abstracted as a Boolean logic node; the fault sets the node to be false, affecting all the functional flows that pass through the node. In fact, AADL-EMV2 supports modeling at exactly all the three levels of abstraction with a slightly different naming system \cite{kushal2017architecture,delange2014architecture}. Obviously, modeling at the function level is more abstract than the architecture level than the component level. 

The semantics dimension is created based on different interpretations of the fault effect. First, the fault effect can be interpreted as a deviation to the intended performance of the defined behavior. In this way, the semantics for the nominal behavior is reused. Second, the local effect is interpreted as a new behavior (such as omission, commission, early, late or value deviations) beyond the original nominal behavior. In this way, only off-nominal states are modeled in the safety model, hence “off-nominal”. Third, the local effect is interpreted as a new off-nominal state but with the ability to interact with the nominal states of the system. In this way, both the nominal states and the off-nominal states are present in the safety model, hence “hybrid”. 
In fact, this semantics dimension is consistent with the classification results of \cite{lisagor2011model-based} that are defined based on the semantics of component interface. 

A detailed classification of a sample set of literature is given in the Appendix. Notably, no literature is found that defines the fault effect in ``(function, nominal)''. In fact, when the fault effect is abstracted as a true/false Boolean value, the nominal performance can only be expressed as ``true'', and the fault effect can only be expressed as ``false''. The semantics does not support the expression of a deviation from the nominal performance. As a result, it is impossible to define the fault effect in ``(function, nominal)'', which is consistent with the classification results in the Appendix.  

\subsubsection{Summary}
We summarize the notable patterns of characterizing the component fault. 
\begin{itemize}
    \item Causal factors:
    \begin{itemize}
        \item Source: The causal factors can come from the external of the component or within the component. The external causal factors can be intended or unintended. 
        \item Occurrence: The occurrence of an external causal factor is ``propagated''. The occurrence of an internal causal factor can be probabilistic or Boolean. 
    \end{itemize}
    \item Activation mechanism: Guard, sequence, delay and duration. 
    \item Impact mechanism: Guard, delay and determinism. 
    \item Effect on component: 
    \begin{itemize}
        \item Semantics: Off-nominal, hybrid, and nominal. 
        \item Abstraction: Function, architecture, and component. 
    \end{itemize}
\end{itemize}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.79\linewidth]{figs/unifying.pdf}
    \caption{The unifying model of component faults.}
    \label{fig:unifying}
\end{figure*}

As a result, the unifying model of component fault can be depicted in Fig.\ref{fig:unifying}. 
The unifying model is summarized from the modeling languages in the literature. 
Such a unifying model not only provides a structure to organize the notable patterns of characterizing the component faults, but also is a generic characterization of how a component fails.  

For the language developers, this unifying model helps them make explicit decisions about what fault phenomenon will be supported by the modeling language and what will not. 
For the safety engineers, the unifying model is language-neutral. The specific patterns presented in the model can be used as guidewords to reason about how the component faults under study actually fail. 
Furthermore, the safety engineers can also use the unifying model to compare different modeling languages, in order to select the most appropriate modeling language for their own problem. 

Finally, although we cannot guarantee the patterns represented in the model are exhaustive, thanks to the flexibility of the basic structure, more patterns can be added to the basic structure as more relevant literature is reviewed. This flexibility allows the authors to keep this unifying model a living artifact and evolve it as we go.

\subsection{Modeling languages selection (Arrow 4)}\label{sec:modeling}
\subsubsection{The modeling languages}
First, the engineering solution is comprised of a set of engineering concepts. The modeling language must be able to represent the engineering concepts that need to be expressed for the engineering solution, which implies an \emph{engineering interpretation} of the modeling language by the domain engineers who generate the engineering solution. Second, different types of analysis require different formalisms. The modeling language must be able to to support the desired analysis, which implies an \emph{formal semantics} of the modeling language that is compatible with the computer programs that conduct the desired analysis. 

For example, a Simulink block has a pre-defined engineering interpretation at the front end to represent the engineering component (e.g., a high-pass filter) and a formal semantics at the back end to support the mathematical analysis. Another example can be something as simple as ``$\int$''. On one hand, ``$\int$'' is a mathematical construct that represents the operation of ``integral''; on the other hand, it can be viewed as an engineering concept that represents the relationship between the acceleration and the velocity. 
In fact, such characterizations of the modeling language are consistent with the concepts of “pragmatic vs. formal” in \cite{batteux2019model}, ``interpretation vs. theory'' in \cite{seidewitz2003models}, and ``abstraction vs. formality'' in \cite{france2007model-driven}.


\paragraph{Modeling.} 
Modeling is to represent the engineering solution with the selected modeling language. As shown in Fig.\ref{fig:language}, the engineering solution and the desired analysis specify what \emph{needs} to be represented and what analysis \emph{needs} to be conducted solely depending on the problem statement. The engineering semantics of the modeling language determines what \emph{can} be represented, and the formal semantics determines what analysis \emph{can} be conducted.  Therefore, a modeling language that fits for the problem statement (1) must be equipped to fully represent the engineering solution and (2) must be analyzable by a computer algorithm for the desired analysis.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/language.pdf}
    \caption{The modeling language must be able to fully represent the engineering solution, and must be analyzable by a computer program for the desired analysis.}
    \label{fig:language}
\end{figure}

Ideally, the modeling process should be conducted in a top-down fashion (Fig.\ref{fig:language}). First, the engineering solution is determined based on the problem statement with no modeling language in mind. Second, the modeling language is selected to fully represent the engineering solution and to support the desired analysis. However, because the modeling language is not considered when the engineering solution is defined, it is possible that no modeling language can be found to represent the engineering solution or some of the desired analysis cannot be conducted with the selected modeling language. 

An alternative approach is bottom-up. As shown in Fig.\ref{fig:language}, the modeling language is selected first to make sure all the desired analysis can be conducted. Then the engineering solution is defined using the selected modeling language. In this way, a model can always be generated. However, a potential problem is that the selected modeling language may not be able to fully express the engineering solution. Especially, if the limitation of the modeling language is not fully understood, the engineers may have unknowingly abstracted important information away from the model even before the analysis is conducted. 

No matter which approach is used for modeling, the engineers must be aware of the limitations of their approach so that they can avoid the potential problems during their own modeling process. 



\subsubsection{Notable patterns}



However, not all modeling language specifies both the engineering interpretation and the formal semantics. We classify the modeling languages into three classes:
\begin{itemize}
    \item Engineering-concept-oriented: They are the modeling languages that focus on representing the engineering concepts without specifying the underlying formal semantics, for example SYSML and Capella \cite{roques2016mbse}.
    \item Formalism-oriented: They are the modeling languages that focus on representing the mathematical operations without a specifying the engineering interpretation, for example Mathematica and Matlab (in .m file). 
    \item Comprehensive: They are the modeling languages that have specified both the engineering interpretations and the formal semantics, such AltaRica 3.0 \cite{prosvirnova2013altarica} and Simulink.
\end{itemize}

\textcolor{red}{SAML}: where does it belong? 
\cite{lipaczewski2015comparison,gudemann2010framework}


Finally, there must be a specific mapping between the engineering interpretation and the formal semantics so that the engineering solution can be transformed into a mathematical model for the analysis by the computer programs. For the ``comprehensive'' languages, such a mapping is usually encoded within the modeling environment so that engineers only need to focus on how to use the modeling language correctly represent the engineering solution. For the ``formalism-oriented'' languages, the engineering concepts are usually represented ad-hoc with the mathematical objects, as the formal semantics can always be assigned with  to represent engineering concepts \cite{rauzy2019foundations}. For the ``engineering-concept-oriented'' languages, one needs to translate it into another modeling language, based on which new computer algorithms can be developed or the existing algorithms can be reused for the desired analysis (e.g., AADL to GSPN \cite{rugina2007system} and UML to Alloy \cite{kherbouche2020formal}).






``The traditional approaches, such as Petri nets, reliability block diagrams, event trees, and fault trees, are models that are very close to mathematical equations and lack structure or lack expressivity power. They also are very abstract compared to the system specification. The model-based safety assessment (MBSA) approaches try to answer these limitations.
The MBSA models have a high expressivity, as they represent systems with a point of view closer to their architecture. The gain on expressive power is obtained by going from Boolean formalisms to state or event formalisms. \cite{vidalie2022category}''


















\subsubsection{Discussion}

\subsection{Safety model construction (Arrow 5)}
\subsubsection{Design view and safety view}
However, the safety model must be constructed in a specific way, otherwise for example the traditional FTA  would be considered as MBSA as the fault tree is generally considered as a safety model. 

It is usually claimed in the literature that MBSA adds value to the current safety engineering practices at the following aspects:
\begin{itemize}
    \item Handling the increasing complexity of safety-critical system.
    \item Integrating the design view and the safety view. 
    \item Finding design shortcomings and flaws early.
    \item Reusing previously developed artifacts.
    \item Introducing automation to reduce time and cost, and improve quality. 
    \item Structuring unstructured information. 
\end{itemize}
In fact, these benefits are also claimed by the general MBD community \cite{scippacercola2016,akdur2018survey,liebel2014assessing,panesar-walawege2013supporting,broy2012what,barbieri2014model-based,jayakumar2020systematic} except the second bullet point: integrating the design view and the safety view. As argued by \cite{barbieri2014model-based}, MBD is just a tool for realizing the integration among the different domain of systems and must be supported by an integrated design methodology. MBSA is exactly such methodology to support the view integration of design and safety. This is also consistent with the claim made by one of the seminal MBSA works \cite{joshi2005proposal} that, MBSA is about maintaining the consistency between the design model and the safety model, and this consistency is unique to MBSA compared with traditional safety analysis.


Obviously, the design model and the safety model are two completely different models. Therefore, the question is, what exactly does the ``consistency'' between the design model and the safety model mean? 









it is the specific ways to implement the global effect subprocess that leads to the consistency between the design model and safety model. The global effect is to model how the fault effect of an individual component affects the system behavior as a whole. While the fault effect of an individual component varies from case to case, the propagation path does have (at least partially) resemblance with the interaction path in the nominal behavior. This resemblance is the basis of the consistency between the design model and safety model. Because the propagation path and the interaction path are the architectures of the safety model and the design model, we call the consistency Architecture Consistency in this paper, and it is one of the defining features of MBSA.





However, the component fault and the local effect subprocesses have no logical consistency with the nominal function of the component, because while the fault of a component might eventually affect the intended function, how it happens and how the fault affects the component are not determined by how the component is supposed to work in the first place. It is worth mentioning that in some works (such as the Generic Failure Model Library [35, 36]), a fault library is developed to associate each component with a fault model. We argue the association is not integration because association is enabled by numerous reuses of the same component in the same (or at least very similar) systems. In fact, the association is a result of MBD approach being able to structure unstructured information and use computer models as media to store institutional knowledge for reuse, i.e. benefit (4) and (6) discussed above.

 

Finally, we are aware there are a handful of works claiming to be MBSA but do not show a clear way to achieve Architecture Consistency, such as [47]. This lack of Architecture Consistency is mainly caused by a loose usage of the terminology by these works. In fact, [47] even defines MBSA as an approach in which the system and safety engineers share a common system model created using a model-based development process, which is consistent with our definition.
\subsubsection{Notable patterns and defining features}




\subsubsection{Discussion}

\subsection{Safety analysis (Arrow 6)}
\subsubsection{Inductive analysis}


\subsubsection{Notable patterns and defining features}
  


 A notable pattern of MBSA is that most works in the literature are the inductive analysis. Note that the inductive analysis is a notable pattern rather than a defining feature, meaning MBSA does not necessarily have to be an inductive analysis. But in this section, we focus on this pattern of MBSA. 

We already knew that an inductive safety analysis is a bottom-up safety analysis. A bottom-up analysis in the context of MBA is, given a set of properties (or requirements) and a model, to verify whether the model satisfies the given requirements. In the context of MBSA, there are generally two types of properties (functional property and safety-critical property) and two types of models (nominal model and off-nominal model). As shown in Fig. \ref{fig:types-induction}, a property-model combination yields 4 types of inductive analysis. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/4_types_analysis.pdf}
    \caption{Four types of inductive safety analysis. The start of the arrow is “verified against” the end of the arrow. No.4 is one of the defining features of MBSA.}
    \label{fig:types-induction}
\end{figure}

Arrow 1 is to verify the “goodness” of the design. The intended function has to be achieved by the designed behavior in nominal conditions. This is the foundation of all other types of analysis. 

Arrow 2 is to verify that the designed behavior in nominal conditions will not lead to hazardous situations. For example, \cite{103} conducted a series of safety assessment to prove that all the possible trajectories of the autonomous cars are not in conflicts by using reachability analysis. 
 
Arrow 3 is to verify the “fail-operational” \cite{126} property of a system design, i.e. the desired function is still achievable even in the case of device malfunction. This is a subject of robustness analysis \cite{127}, a dependability property that is closely related to safety. 

Arrow 4 is to verify the fail-safe property.  As explained in the previous section, this is one of the minimal requirements for any work to be considered as MBSA.  

While there are many types of causal factors such as design error, manufacture defect, human error and component failure, a minimal requirement for a safety analysis is that it must address component failure. In other words, the goal of a safety analysis must at least involve proving the system is fail-safe. This is a defining feature that MBSA at least has to be able to argue whether a system is fail-safe. In fact, most MBSA works focus on modeling component failure with an exception of the EAST-ADL framework \cite{24, 25}, where the process faults (systematic faults such as design, implementation, installation, operation and overstress faults) are considered in the modeling semantics. However, it is unclear from the literature how process faults are identified, mitigated and implemented by the framework.


It is worth mentioning that all the four arrows can be implemented by a {\bf Formal Methods}. In Model Checking \cite{lindsay2010model}, a safety property is even explicitly defined in the methodology. However, if a formal analysis does not include Arrow 4, it is not MBSA, even if a safety-critical property is verified against. 

\subsubsection{Discussion}

\subsection{The defining features of MBSA}
The defining feature is to model the propagation. Not vertical causation, but horizontal causation, or propagation, or flow, or component dependency, or interaction. 


==> 5_case.tex <==
\section{A case study}\label{sec:case}
FTA is not formally related to the technical architecture of the system \cite{kaiser2018advances}.



==> Z_bio.tex <==
\bio{}
Author biography without author photo.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
\endbio

\bio{figs/pic1}
Author biography with author photo.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
\endbio

\bio{figs/pic1}
Author biography with author photo.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
\endbio

==> copy_2_background.tex <==
\section{Background}\label{sec:background}

The MBA process described in this paper is derived from the MBD process, as MBA itself is not a widely used concept. In this section we start with MBD to provide a context for MBA and then zoom in to MBA to further provide a context for MBSA later.


\subsection{The MBD process}
First of all, we are aware that MBD is an overloaded term, as numerous papers tried to differentiate it from ``model-driven engineering'', ``model-driven design'' and ``model-driven architecture'' \cite{104,105}. It is not our intention to define these terms. However, we need a clear understanding of MBD to conduct meaningful discussion about the body of literature pertaining to (or not pertaining to) MBSA. Hence, we adopt the process proposed by \cite{106} as the “ground truth” of our discussion. The left of the Fig.1 is the proposed MBD process which can be mapped to the detailed 10 steps of \cite{106} at the right. Two loops, an inner loop and an outer loop, are identified for the MBD process. We explain all the involved steps in this section and will zoom in on the inner loop in the next section. 

 
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figs/mbd_process.pdf}
    \caption{The MBD process. The arrows of the left can be mapped to the steps to the right (adopted from \cite{106}). The inner loop (shaded area) is the model-based analysis. }
    \label{fig:mbd_process}
\end{figure}


An MBD process starts with a problem statement (Step A) which details the goal of the design activities, such as a set of functions with performance requirements and safety constraints. 
Second, an engineering solution is derived based the engineer’s domain knowledge. Although 3 independent steps (Step B, C, D) are identified by \cite{106}, we acknowledge this process in reality can be quite fuzzy, because the engineer’s thought process varies from person to person, depending on their own expertise and nature of the problem at hand. Nevertheless, we prescribe the process always ends with a solution (valid or not) to the stated problem from the perspective of the specific engineering discipline. 
Third, a modeling language is selected to faithfully represent the engineering solution with a model of computation (Step E). Compared to a simulation model that is to loosely ``get a feel'' of the proposed engineering solution, the model in MBD is a faithful computational copy of the engineering solution and hence used as the primary artifact \cite{114}. Models in MBD are directly evolved into full-fledged implementations without changing the engineering medium, tools, or methods \cite{107}. Specifications and even software code of the implementation are (automatically) derived from the model \cite{108, 134}. Therefore, the modeling language must be fully equipped to express the engineering solution.  

Fourth, the model of computation is automatically analyzed to gain a required level of confidence of the engineering solution before building the prototype or the real system (Step G). This step closes the inner loop. Analysis techniques with different level of mathematical rigor such as simulation and formal methods, are usually required in accordance with the required level of confidence. Obviously, this not only begs the question of the availability of the tool support for the analysis, which itself is an entire research area, but also whether the semantics of the modeling language can be formalized in a way that tools can be developed for the desired automated analysis. 

Fifth, specification is derived from the model of computation (Step F); hardware is constructed in accordance with the specification (Step H); software is developed or automatically generated from the model and synthesized with the hardware (Step I). This is what makes the “model” in MBD different from models for simulation, because 1) specifications for constructing a prototype of the real system are derived from the model, for example a CATIA model can be used for both structural analysis and directly as 3D drawings for manufacture \cite{110}, and 2) software code sometimes can even be automatically generated from it, which is the perhaps the main reason for MBD’s growth of popularity in the first place \cite{111}.    

Finally, Step J closes the outer loop. The prototype or the real system is verified, validated and tested against the problem statement made at the beginning of the MBD process. 
Clearly, as shown in Fig. 1, an MBD process consists of an inner loop and an outer loop, where the former is about modeling and analysis, and the latter is about construction (automated or not) and testing.  As defined by \cite{112}, a hazard analysis is “the process of identifying hazards and their potential causal factors”. Although it is a highly iterative process, meaning verification is still required after the construction (e.g. the SSA process of \cite{113}), the hazard analysis mostly happens during the inner-loop so that safety-critical decision can be made early before construction of the prototype or the real system. 
Therefore, for MBSA, we mainly focus on the inner loop, which is the shaded area in Fig.1, and we call this inner loop ``Model-based analysis'' (MBA).


\subsection{The MBA process}
In this section, we take a closer look at the inner loop of Fig.1 to derive a more general MBA process. As shown in Fig. 2, the artifacts at the righthand side is adopted from Fig. \ref{fig:mbd_process}. The activities to generate these artifacts are expressed in more general terms and the supports for the activities are displayed at the left-hand side, both of which will be explained in great details in this section.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/artifacts.pdf}
    \caption{The MBA process, where the artifacts of the righthand side are adopted from the inner loop of Fig. \ref{fig:mbd_process} and the left-hand side are the supports for the respective activities. }
    \label{fig:mba_process_artifacts}
\end{figure} 


First, from the perspective of an application engineer, the MBA process consists of three steps: ``formulate'', ``express'' and ``analyze'' (the right workflow in Fig. \ref{fig:mba_process_artifacts}).

\paragraph{Step 1}: given a design problem, the engineers first use their domain knowledge to “formulate” an engineering solution to that problem. Informally, the engineering solution is the engineer’s understanding of the real behavior of the system-to-be-built and his/her decisions about what to capture from this "real" behavior by applying his/her domain knowledge. Although the resulting engineering solution has eventually to be represented in a certain modeling language and any modeling language has a limit of expressiveness, in theory this “formulate” process has to be language-neutral, meaning solely determined by applying the domain knowledge, not limited by the modeling language. For example, the engineering solution of a control system should solely be determined by the physical dynamics and preferred control policy rather than the modeling language such as Matlab and Modelica.

However, in reality, this “formulate” process is more complicated. As explained in Section 2.1 about MBD, because primary artifacts such as specification, software code and safety decision are made from this process, the engineering solution has to be faithfully represented by the model of computation, meaning the modeling language has to be fully equipped to express the engineering solution. Two possibilities exist for this concern. One is to find the appropriate modeling language after the engineering solution is developed or design a new modeling language if none of the current ones fits; the other is to have one or multiple candidate modeling languages in mind beforehand, use the modeling languages to “formulate” the engineering solution, and finally pick the most appropriate one. In reality, for most engineers who use models to develop their own systems, the latter is most dominant. In fact, the structured semantics of a modeling language can help engineers to perceive the problem and manage the cognitive complexity in the problem-solving process. 

This observation has a significant implication because although the “formulate” process focuses on problem solving and highly relies on the domain knowledge, the resulting engineering solution has to be practical enough so that it can be expressed by a modeling language. Hence, two “support” arrows (Fig. 2) from the domain knowledge and the language semantics go into the engineering solution. We make the following assertion, which is similarly referred as “the abstraction challenge” in \cite{107}.

\paragraph{Assertion 1}: The modeling language, especially its semantics, has to be able to represent the engineering solution.

\paragraph{Step 2}: the engineering solution, already consistent with the semantics of the modeling language, is mapped accordingly to the language syntax and eventually yields the model of computation. We call this process “express” because it is simply a “faithful” representation of a well formulated engineering solution (in whatever form) to a well-defined explicit model in the computer. Note that, this process is only to “express”. Information shall neither be subtracted from the engineering solution nor added to it.

\paragraph{Step 3}: the model of computation is “analyzed” automatically, so that a required level of confidence can be established. Specifically, different levels of confidence require different analysis techniques such as step-wise trace demonstration, stochastic simulation and model checking, which in turn has an implication on the formalism of the modeling language. In other words, analysis techniques must be available for the desired analysis with the selected language, thus an arrow from the “semantics” to the “analysis” in Fig. 2. Therefore, we make the following assertion, which is similarly referred to as “the formality challenge” in \cite{107}. 

\paragraph{Assertion 2}: The modeling language, especially its semantics, has to be analyzable by computer programs for the desired analysis. 

From the perspective of the methodological support (the left workflow in Fig. \ref{fig:mba_process_artifacts}), it includes language support and tool support. The modeling language, particularly its semantics, has to be expressive enough to fully represent the engineering solution (Assertion 1) and techniques and tools must be developed for the modeling language for the desired analysis (Assertion 2). Obviously, the semantics of the modeling language plays a center role here. As shown in Fig. 3, it affects the formulation of the engineering solution (the upper loop) and the feasibility of the desired analysis (the lower loop). 

For language support, we further assert that the semantics of a modeling language in the MBA process must simultaneously have a {\em context-specific} {\bf modeling construct} for the engineer to represent the engineering solution (the upper loop) and a {\em context-free} {\bf mathematical construct} for the computer to conduct the desired analysis (the lower loop). For example, a Simulink block at the same time has both a specific engineering meaning at the front end and a context-free purely mathematical expression at the back-end, such as a high-pass filter has a modeling construct that means signals below a cutoff frequency are attenuated and a mathematical construct that is usually represented by a first-order mathematical transfer function. The transition in a Markov process can mean at the same time both the triggering of a failure event (i.e. the modeling construct) and a context-free Poisson process (i.e. the mathematical construct).  In fact, the modeling construct and the mathematical construct are consistent with the concept of “pragmatic model” and “formal model” in \cite{15}. The difference is that modeling construct and mathematical construct are two aspects of the same model rather two different types of model as argued in \cite{15}.

There is usually a unique mapping between the modeling construct and the mathematical construct, to translate between the context-specific concepts and the context-free mathematical expression. Depending on the specific situations, this translation is bi-directional. The engineer can use an appropriate modeling construct directly to “formulate” the engineering solution, such as modeling in Simulink. The resulting model is translated (usually automatically by the modeling environment) into the context-free mathematical model (i.e. the downward translation) for the desired analysis later. It is also possible the engineer uses the mathematical construct directly to “formulate” the engineering solution, such as writing state space model in a Matlab file, he/she then needs to reconstruct the modeling construct (i.e. the upward translation) manually from the mathematical construct to link with the context-specific concepts, in order to make sure the resulting mathematical model faithfully represents the solution in the specific engineering context. It is worth mentioning that it can very difficult to “formulate” the engineering solution directly with the mathematical construct especially for complex systems, because the manual mathematically modeling for complex system is error prone and the resulting model in pure math is very difficult to communicate and review, which is why modeling with Simulink has gained much more traction than modeling directly with Matlab script files. Hence, the upward translation is not considered for the rest of the paper. 

For tool support, algorithms are developed around the mathematical construct of the modeling language for the desired analysis. Sometimes in order to reuse existing algorithms, “model transformation” algorithms such as AADL to GSPN \cite{115} are developed to translate the mathematical construct of the current modeling language to the formalism that the target algorithms can be applied to. 

Although algorithms can be developed for the desired analysis or model transformation, an inappropriate abstraction level of the modeling language can render the desired analysis infeasible. For example, a traditional fault tree cannot generate the critical event sequence for a top-level event, simply because the sequence information is abstracted by the semantics of the traditional fault tree. More information has to be included (hence less abstract), such as the Dynamic Fault Tree \cite{16, 17}, for the desired analysis. This echoes our previous claim that the semantics of the modeling language not only affect the formulation of the engineering solution, but the feasibility of the desired analysis.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/semantics.pdf}
    \caption{The semantics of the modeling language is at the center of an MBA process in the view of a methodology developer.}
    \label{fig:semantics}
\end{figure} 


To conclude, Table 1 is a summary of the MBA process. From the perspective of the domain engineer, the process mainly consists of three activities: “formulate”, “express” and “analyze”. Each of the activities requires different methodological supports, which are essentially application and manipulation of the “modeling construct”, “mathematical construct” and “syntax” of the modeling language. 

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|p{0.8in}|p{0.8in}|}
        \hline
        \multicolumn{2}{|c|}{\multirow{2}{*}{Domain engineer}} &	 \multicolumn{2}{c|}{Methodology developer} \\ \cline{3-4}
        \multicolumn{2}{|c|}{} & Language support &	Tool support \\ \hline
        \multirow{2}{*}{Manual} &	Formulate	& Modeling construct &	NA \\ \cline{2-4}
        & Express &	Syntax to express the engineering solution &	Modeling environment  \\ \hline
        \multirow{2}{*}{Automated} &	\multirow{2}{*}{Analyze} &	Mathematical construct to be translated. &	Programs for model transformation \\ \cline{3-4}
		& & Mathematical construct to be analyzed. &	Programs for the desired analysis  \\ \hline
    \end{tabular}
    \caption{The summary of the MBA process.}
    \label{tab:summary}
\end{table}



Finally, we focus this paper on how the modeling language supports the MBSA process rather than how the modeling language is supported and implemented by tools, as the former is closer to System Safety Engineering community while the latter is mostly Software Engineering. For this reason, we adapt the MBA process of Fig. \ref{fig:semantics} into Fig. \ref{fig:language_support} below, with a more explicit depiction of the relationship between the MBA process and the modeling language. The rest of the paper will follow closely with Fig. \ref{fig:language_support}. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/language_support.pdf}
    \caption{The MBA process and the language support. While the analytical process represents a series of (iterative) steps [right], it is supported by particular choices with respect to the modeling language [left]. The discussion of MBSA will follow closely with this process. }
    \label{fig:language_support}
\end{figure}


==> modeling.tex <==
\section{Model, modeling language and modeling}\label{sec:model}
We explain the concepts of ``model'', ``modeling language'' and ``modeling'' in the context of MBD. These concepts might have different meanings in other contexts because they may follow different processes and serve different goals.   We will use these concepts to reason about MBSA in Section \ref{sec:MBSA}.   

\paragraph{Model.} Model is the same as the ``model of computation'' in MBD. It resides in a computer,  represents the engineering solution, and supports a set of the desired analysis that can be conducted automatically by a computer program. 

\paragraph{Modeling language.}
First, the engineering solution is comprised of a set of engineering concepts. The modeling language must be able to represent the engineering concepts that need to be expressed for the engineering solution, which implies an \emph{engineering interpretation} of the modeling language by the domain engineers who generate the engineering solution. Second, different types of analysis require different formalisms. The modeling language must be able to to support the desired analysis, which implies an \emph{formal semantics} of the modeling language that is compatible with the computer programs that conduct the desired analysis. 

For example, a Simulink block has a pre-defined engineering interpretation at the front end to represent the engineering component (e.g., a high-pass filter) and a formal semantics at the back end to support the mathematical analysis. Another example can be something as simple as ``$\int$''. On one hand, ``$\int$'' is a mathematical construct that represents the operation of ``integral''; on the other hand, it can be viewed as an engineering concept that represents the relationship between the acceleration and the velocity. 
In fact, such characterizations of the modeling language are consistent with the concepts of “pragmatic vs. formal” in \cite{batteux2019model}, ``interpretation vs. theory'' in \cite{seidewitz2003models}, and ``abstraction vs. formality'' in \cite{france2007model-driven}.


\paragraph{Modeling.} 
Modeling is to represent the engineering solution with the selected modeling language. As shown in Fig.\ref{fig:language}, the engineering solution and the desired analysis specify what \emph{needs} to be represented and what analysis \emph{needs} to be conducted solely depending on the problem statement. The engineering semantics of the modeling language determines what \emph{can} be represented, and the formal semantics determines what analysis \emph{can} be conducted.  Therefore, a modeling language that fits for the problem statement (1) must be equipped to fully represent the engineering solution and (2) must be analyzable by a computer algorithm for the desired analysis.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/language.pdf}
    \caption{The modeling language must be able to fully represent the engineering solution, and must be analyzable by a computer program for the desired analysis.}
    \label{fig:language}
\end{figure}

Ideally, the modeling process should be conducted in a top-down fashion (Fig.\ref{fig:language}). First, the engineering solution is determined based on the problem statement with no modeling language in mind. Second, the modeling language is selected to fully represent the engineering solution and to support the desired analysis. However, because the modeling language is not considered when the engineering solution is defined, it is possible that no modeling language can be found to represent the engineering solution or some of the desired analysis cannot be conducted with the selected modeling language. 

An alternative approach is bottom-up. As shown in Fig.\ref{fig:language}, the modeling language is selected first to make sure all the desired analysis can be conducted. Then the engineering solution is defined using the selected modeling language. In this way, a model can always be generated. However, a potential problem is that the selected modeling language may not be able to fully express the engineering solution. Especially, if the limitation of the modeling language is not fully understood, the engineers may have unknowingly abstracted important information away from the model even before the analysis is conducted. 

No matter which approach is used for modeling, the engineers must be aware of the limitations of their approach so that they can avoid the potential problems during their own modeling process. 
